Learning to Price Homogeneous Data

We study a data pricing problem, where a seller has access to $N$ homogeneous data points (e.g. drawn i.i.d. from some distribution). There are $m$ types of buyers in the market, where buyers of the same type $i$ have the same valuation curve $v_i:[N]\rightarrow [0,1]$, where $v_i(n)$ is the value for having $n$ data points. A priori, the seller is unaware of the distribution of buyers, but can repeat the market for $T$ rounds so as to learn the revenue-optimal pricing curve $p:[N] \rightarrow [0, 1]$. To solve this online learning problem, we first develop novel discretization schemes to approximate any pricing curve. When compared to prior work, the size of our discretization schemes scales gracefully with the approximation parameter, which translates to better regret in online learning. Under assumptions like smoothness and diminishing returns which are satisfied by data, the discretization size can be reduced further. We then turn to the online learning problem, both in the stochastic and adversarial settings. On each round, the seller chooses an anonymous pricing curve $p_t$. A new buyer appears and may choose to purchase some amount of data. She then reveals her type only if she makes a purchase. Our online algorithms build on classical algorithms such as UCB and FTPL, but require novel ideas to account for the asymmetric nature of this feedback and to deal with the vastness of the space of pricing curves. Using the improved discretization schemes previously developed, we are able to achieve $\tilde{O}(m\sqrt{T})$ regret in the stochastic setting and $\tilde{O}(m^{3/2}\sqrt{T})$ regret in the adversarial setting.

==> Appendices/A_related_work.tex <==
\section{Related work}\label{app:related_work}
\textbf{Dynamic pricing}. The online posted-price mechanism, also known as dynamic pricing, is a central research area in algorithmic market design~\cite{kleinberg2003value, den2015dynamic}. In the most classical setting~\cite{kleinberg2003value}, the seller sets a price for an item in each round, and a buyer purchases the item only if their valuation exceeds the posted price. While several extensions of this setting have been explored for both parametric~\cite{keskin2014dynamic,den2014simultaneously,besbes2015surprising,javanmard2017perishability,javanmard2019dynamic,xu2021logarithmic} and non-parametric~\cite{besbes2009dynamic,wang2021multimodal,cheung2017dynamic,misra2019dynamic,perakis2023dynamic} demands, most focus on single-parameter demands, i.e., selling a single item to buyers. Our data pricing problem is multi-parameter, as demands are parameterized by multiple outcomes, i.e. the number of data points.

\textbf{Bayesian unit-demand pricing problem}. Formally, our data pricing problem is a variant of the Bayesian Unit-demand Pricing Problem (BUPP)~\citep{chawla2007algorithmic}. BUPP addresses the problem of (offline) revenue maximization over a known distribution of unit-demand buyers, meaning they want to buy at most one item from the inventory. In BUPP, a seller has $\numdata$ distinct items to sell to a unit-demand buyer whose valuations are $v=(v_1,\dots,v_\numdata)$, where $v_i$ is the value of the $i$th item. Given prices ${p_i}{i\in [\numdata]}$, the unit-demand buyer purchases a single item $i\in[\numdata]$ that maximizes their utility: $v_i - p_i$. Assuming the valuation profile $v$ follows a known distribution $D$, the goal of BUPP is to find the best prices ${p_i}_{i\in [\numdata]}$ that maximize the seller's expected revenue.
    
Our data pricing problem is a variant of BUPP in two ways: \emph{(1)} We study the sequential setting where type distributions are \emph{unknown}, while valuation profiles for each type are known, and \emph{(2)} We assume monotonic values $v_1 \leq \dots \leq v_\numdata$, which is natural in data pricing. Unfortunately, BUPP is a computationally intractable problem, as is ours. BUPP is known to be \textsf{NP}-hard even when $D$ is a product distribution~\citep{chen2014complexity}. Moreover, even assuming that values are monotonic (i.e., $v_1 \leq \dots \leq v_\numdata$), the problem remains (strongly) \textsf{NP}-hard~\citep{chawla2022pricing}. Therefore, we aim to provide a reasonably efficient no-regret algorithm for our problem, especially when the number of types $\numtypes$ is a fixed constant.

\textbf{Market design for data-sharing}. In recent years, there has been a plethora of work devoted to algorithmic market design for data sharing~\citep{agarwal2019marketplace, agarwal2020towards, jia2019towards, wang2020principled}. These works provide ingenious solutions to challenges unique to the data market, such as free replicability and the difficulty of valuation due to the combinatorial nature of data. Except for~\citet{agarwal2019marketplace}, the above-cited solutions are inherently \emph{offline or single-shot}. While we focus on a simplified yet relevant setting where data comes from a single source, resulting in monotonic valuations, in this work, we tackle the problem in a sequential, dynamic setting, which has practical importance.
In contrast to our approach, \citet{agarwal2019marketplace} considered the price to be a constant (i.e., a scalar rather than a price vector) to address the inherent computational intractability of multi-dimensional pricing. Instead, we maintain the price as a vector (i.e., a price function) but focus on cases where the valuation function satisfies natural properties such as monotonicity, smoothness, and diminishing returns.
